The Ratio of Helium- to Hydrogen-Atmosphere White Dwarfs: Direct Evidence for Convective Mixing

We determine the ratio of helium- to hydrogen-atmosphere white dwarf stars as a function of effective temperature from a model atmosphere analysis of the infrared photometric data from the Two Micron All Sky Survey combined with available visual magnitudes. Our study surpasses any previous analysis of this kind both in terms of the accuracy of the Teff determinations as well as the size of the sample. We observe that the ratio of helium- to hydrogen-atmosphere white dwarfs increases gradually from a constant value of ~0.25 between Teff = 15,000 K and 10,000 K to a value twice as large in the range 10,000 > Teff > 8000 K, suggesting that convective mixing, which occurs when the bottom of the hydrogen convection zone reaches the underlying convective helium envelope, is responsible for this gradual transition. The comparison of our results with an approximate model used to describe the outcome of this convective mixing process implies hydrogen mass layers in the range log M_H/M_tot = -10 to -8 for about 15% of the DA stars that survived the DA to DB transition near Teff ~ 30,000 K, the remainder having presumably more massive layers above log M_H/M_tot ~ -6.

==> response <==

                                                  September 12th, 2007
Dear Dr. Pipher, 

Please find below the revised electronic version of our paper
entitled:

"The Ratio of Helium- to Hydrogen-Atmosphere White Dwarfs: Direct
Evidence for Convective Mixing"

by P.-E. Tremblay and P. Bergeron, submitted to the Astrophysical
Journal.

We would like to thank the anonymous referee for a careful reading of
our manuscript and for his/her constructive comments, which have all
been taken into account in our revised version. We described below the
changes made. We hope that these changes will be acceptable to both
you and the referee.

All correspondence should be sent to:

        Pier-Emmanuel Tremblay
        Department of Physics
        University of Montreal
        2900 boul. Edouard-Montpetit
        Montreal, Quebec
        Canada H3T 1J4

        e-mail: tremblay@astro.umontreal.ca
        Phone : (514) 343-6111 X-1089
        FAX:    (514) 343-2071

Files submitted:

  README      This file

  ms.tex      Manuscript file
  ms.aux      Auxiliary file for cross-references

  tab1.tex    Table 1
  tab2.tex    Table 2

  f1.eps      This file and following are Figure files
  f2.eps
  f3.eps
  f4.eps
  f5.eps
  f6.eps
  f7.eps
  f8.eps
  f9.eps
  f10.eps
  f11.eps

-----------------------------------------------------------------------

We would like to thank the anonymous referee for a careful reading of
our manuscript and for his/her constructive comments, which have all
been taken in the changes described below.

> This paper confirms in a more quantitative way a result that non-DA/DA
> ratio increases below 10,000K due probably to hydrogen convection.
> The Sion (1984) study, by necessity, used his sample in a less
> uniform or homogeneous manner of Teff estimate than this study.

We beg to differ with the referee on this issue. The Sion (1984)
analysis has been cited over and over again as evidence for a change
in the ratio of DA to non-DA stars at low effective temperatures, but
as already criticized in Bergeron, Wesemael, Fontaine, & Liebert
(1990, ApJ, 351, L21) and more explicitly in our Introduction and
particularly in our Figure 2, the evidence based on the statistics of
Sion (1984) are not compelling *at all*. So our results are not a
simple confirmation of a result we already knew.

> There are, however, flaws in the way the present study is done.
> Nonetheless, if the authors can address the points raised in this
> report, especially the log g = 8 question, I think the paper can
> probably be recommended for publication.

We find the word "flaws" a bit harsh since our analysis is infinitely
superior to that of Sion (1984), which was based on empirical Mv
calibrations and nothing else. We actually went to a great deal to
explore all possible systematic effects, none of which were even
remotely considered in the Sion analysis. We would prefer to call
those "limitations" rather than "flaws", and we have tried to address
these unavoidable limitations carefully in Section 4 and in our reply
below.

> Introduction:
> 
> Where do the magnitude thresholds quoted of J~ 16.8, H 16.5 and K_S 16.2 
> come from? 
> Skrutskie et al 2006 AJ, 131, 1163 is the definitive description of the 
> final 2MASS products.  The project's conservative goals were to achieve 
> 10 sigma detections to J,H,K  = 15.8, 15.1, 14.3 respectively.  This 
> paper demonstrates that these goals were handsomely exceeded -- see, 
> for instance Table 2 and Figure 16.  But the numbers quoted by the 
> authors seem unrealistically faint.  I think the answer is that the 
> authors do not need 10 sigma accuracies.  The tests performed using 
> the photometry to compare temperature determinations with other 
> methods indicate that they are probably on sound ground. 

These magnitudes thresholds are for detections of any accuracy -- see
Fig. 1 of Tremblay & Bergeron (2007, ApJ, 657, 1013). Hence they are
much lower than the 10 sigma detection limits quoted in Skrutskie et
al. (2006). Indeed, our analysis has shown that we do not need to
restrain to the 10 sigma sample because the temperature uncertainties
for most objects are well below those required in our analysis (1000 K
and 2000 K bins). We have clarified the magnitude thresholds quoted in
our manuscript in the following way:

   "...magnitude thresholds of J~16.8, H 16.5, K_S 16.2 for detections 
    with any formal uncertainty (see for instance Fig.~1 of Tremblay 
    & Bergeron 2007)"

> "tend to float" -- I would remove the "tend to" 

Done.

> "the DA stars .. with presumably hydrogen-dominated atmospheres"? 
> Hasn't this been amply proven?  Delete "presumably".  

We have deleted the "presumably" but below 10,000 K, it is not clear
at all whether DA stars have atmospheres dominated by hydrogen.

> "multiple excursions on the AGB nuclear burning phase" [which they 
> say could cause additional ejection of hydrogen envelope below 
> the canonical 10^-2].  What does this phrase mean?  Helium shell 
> flashes?  especially a very late one which could remove essentially 
> all of the hydrogen.  I think the phrasing is too vague as is. 

We have clarified the sentence and added a reference

   "However, multiple excursions on the AGB nuclear burning phase, during 
    which very late helium flashes could remove essentially all of the 
    hydrogen (Werner & Herwig 2006),..."

> "It is generally believed..turning all helium-atmosphere white dwarfs 
> into DA stars" 
> I would amend this to say something like
> "It has traditionally been believed"   
> since the recent Sloan discovery shows that this was not correct. 

Done. Indeed it is now clear that not all helium-atmosphere white
dwarfs turn into DA stars. We mention this in our paper but further
below.

>  Section 2:
> 
>  Why does the DA curve in Figure 3 turn over below 5,000K?  Well, its due
>  to the CIA opacity.  Perhaps this should be mentioned in the figure
>  caption since it looks strange, though irrelevant to the paper after the
>  Teff cut of 5,000K is applied.

We have added the following sentence in the caption:

   "The turnover of the hydrogen-atmosphere curve below 5000 K is due to the 
    onset of the collision-induced absorptions by molecular hydrogen."

>  Section 3: 
>  
>  p. 6: "weak DA stars such as Ross 640" and used a second time --   
>  these are normally classified DZA in the Sion et al. (1983) 
>  system, and "DZA" is actually used later in the paper 

Here we meant cool white dwarfs with a helium dominated atmosphere and
a trace of hydrogen. we have clarified our sentence as follows:

   "...helium-atmosphere objects with weak hydrogen features such as Ross 640"

and then on p.10:

   "--- either DQ, DZ (or DZA), or DC ---"

>  Figure 4's ups and downs look strange, though small enough excursions
>  probably not to matter.  Maybe a sentence or two about why this behavior
>  is appropriate.

These curves are basically the derivative of a magnitude with respect
to log g (here it is the V-J color index but a curve of V would be
very similar). The magnitudes as a function of effective temperature
have a slightly different slope for different values log g, mainly due
to the fact that the various opacity sources peak at slightly
different temperatures. This results in the ups and downs in the 
d (V-J) / d log g function. We have added the following sentence in the
figure caption:

   "The general behavior of these curves can be explained in terms of the 
    various opacity sources that peak at slightly different effective temperatures
    for these two $\log g$ values."

>  "the mass distributions of hydrogen- and helium-atmosphere white dwarfs
>  are to a good approximation identical" 
>  this is not correct -- the mean masses are identical within the
>  uncertainties, but the DA mass distribution is now known to have many
>  more low and high mass outliers than do the DBs (Beauchamp thesis, but
>  also Voss et al. 2007 A&A, 470, 1079).  The vast majority of DB stars
>  are log g near 8, but what bias will the DA outliers cause to the
>  statistics?

We are aware of this fact, which was also mentioned in a similar
analysis of hot DB stars made by Eisenstein et al. (2006, AJ, 132,
676). In terms of determining the effective temperatures based on
*photometry*, we have clearly shown in our Figure 4 that the value of
log g we adopt does not have a significant impact on our temperature
determinations, even for log g values +/-0.5 dex from the mean. In
other words, the energy distributions are not particularly log g
sensitive (especially if one neglects the U filter, as we did, which
measures the strength of the Balmer jump). The main point we were
trying to make is that a mean value of log g is equally valid for DA
and DB stars. We have modified our sentence to be more specific:

   "Since the mass distributions of hydrogen- and helium-atmosphere 
    white dwarfs have to a good approximation the same mean value (...),
    this simplifying assumption should not affect the results of our 
    analysis significantly." 

Also, the results of Voss et al. (2007) for the mass distribution of
DB and DBA stars in the SPY project indicates a much broader peak than
found by Beauchamp, in much better agreement with the results for the
DA stars. So it is no longer true that the number of outliers in the
mass distribution of DB stars is small, at least according to Voss et
al. (see below also).

> In a magnitude limited survey as this essentially is, the low mass /
> large radius DA component will be over-represented relative to a fixed
> volume of space.  It is possible that the systematic error may be fairly
> small, but should at least be acknowledged.  If Liebert, Bergeron and
> Holberg's analysis can be used to quantify this, perhaps this can be
> added.

Indeed, this effect could be important in terms of the volume effect of
our Figure 10. We have added the following discussion in Section 5:

   "While the assumption of a fixed value of $\log g$ was appropriate for
    determining the effective temperatures, this may not be the case for
    the volume effect discussed here. Indeed, white dwarfs stars with
    large radii (or low masses) can be detected at larger distances. The
    differences in the mass distributions of DA and DB stars could
    therefore affect the ratio \citep[see also][]{eisenstein06a}. While
    the results of \cite{beauchamp96} suggest that the mass distribution
    of DB stars is narrower than that of DA stars, the recent results of
    \citet{voss07} reveal instead that both distributions are comparable.
    Hence the small residual differences in the low and high mass tails
    are not expected to affect our results significantly."

> excluding 90 binaries would bring the sample size down to 850, if I have
> followed the sequence of steps.  However, the Teff cuts leave just 447
> (Section 5).  Perhaps this should be more explicitly stated. 

Good point. We have clarified these numbers in the following way:

   "...for our final 2MASS sample of 447 objects (after the temperature 
    cutoff at Teff=15,000 and 5000 K and the removal of 2MASS data with low
    accuracy above Teff=11,000 K have been applied)."

>  Section 4: 
>  
>  18 DB stars with Teff determined spectroscopically -- 
>  the appropriate reference is Beauchamp 1995 (thesis) 
>  as I don't think these numbers are given in the short conference 
>  proceeding -- Beauchamp et al. 1996 
>  One would like to see these parameters published in a refereed 
>  journal, or an updated analysis.  

We have added both references since the Beauchamp (1995) PhD thesis
includes only half of the DB stars analyzed in Beauchamp et al. (1996).
Publications of these parameters in a refereed journal is underway,
and has been complicated by the fact that Alain Beauchamp has left the
field of astronomy several years ago.

> Section 5: 
> 
> Figure 10 -- another strange looking curve 
> this is all due to opacities no doubt 
> but why does the ratio climb to 1.25 near 20,000K 
> then fall to 0.9 below 10,000K? 
> It zooms below 5,000K of course because of the CIA opacity. 

The volume ratio V_He/V_H is proportional to f_nu_He/f_nu_H ** 3/2.
Here we use the H-band flux but the standard V-band flux would yield
similar results. As stated in Eisenstein et al. (2006), these flux
differences are due to opacities. We find these are mainly continuum
opacities such as H-, He- and bound-free opacities, although there is
not much literature about continuum opacities for DA and DB around
20,000 K. We have added modified our sentence for completeness:

   "However, this distance is different for hydrogen- and helium-atmosphere 
    white dwarfs because they have different continuum opacity sources and 
    corresponding monochromatic fluxes."

> An aside: the non-DA mass distribution may pick up some massive DA
> converts below 10,000K.  If losing most of the hydrogen on the AGB is
> due to helium shell flashes, well stellar evolution work shows that
> these are more frequent and perhaps violent around a massive core.  So
> the result may be a DA star with < 10^-6 mass hydrogen, which converts
> to a non-DA below 10,000K.  The only way to find such cases may be
> through trig parallaxes.

This is an interesting theory. One would have to first identify or
confirm which cool helium-atmospheres objects are converts. If these
are indeed the DZA as suggested by Dufour et al. 2006, it would be
interesting to compare their mean masses.

> "The results of Dufour et al. (2005,2006) reveal that photometric 
> temperature of DQ and DZ stars can be systematically reduced by 500K on 
> average..."
> 
> True, but only for low Teff stars. As Teff gets higher, the temperature
> shifts get bigger and bigger. For example, Wegner & Koester 1985 find
> that for the DQ G227-5, T(He)=18,000 K while T(with carbon)=12,500 K. This
> shift is certainly not negligeable for DQs. They are however relatively
> rare and the present result is probably not affected by this. 

We were aware of this result but we do not have any star in our sample
classified as DQ with temperatures much higher than 10,000 K, which is
about the upper limit of the Dufour et al. analyses.

> But how DBs with undetected amounts (in the visible) of carbon can be
> affected is practically unexplored. UV observations of DBs seem to
> show that they do contain traces of carbon (Petitclerc et al.). But
> by what amount and how exactly it affects the Teff determination for
> those between 20,000 and 12,000K is uncertain. This is a possibility
> that perhaps needs to be considered when discussing the
> Helium/Hydrogen ratio in the 14,000-12,000K bins.

This is true but this source of uncertainty has already been
acknowledged in our paper (note that we have now added explicitly the
word "carbon"):

   "The numbers given above could change slightly if one takes into
    account the presence of traces of metals (including carbon) and
    hydrogen in the model atmosphere calculations of DQ and DZ
    stars. Indeed, the atmospheric structure of cool helium-atmosphere
    white dwarfs is affected significantly by small traces of metals or
    hydrogen, which then provide most of the free electrons
    \citep{provencal02, dufour05, dufour07}. These additional electrons
    increase the contribution of the He- free-free opacity, which in
    turn reduces the atmospheric pressure.  The results of Dufour et
    al. (2005, 2007) reveal that photometric temperatures of DQ and DZ
    stars can be systematically reduced by 500 K on average when metals
    are included in the model calculations.  Therefore, this could affect
    the precise temperature dependence of the change in the ratio of
    helium- to hydrogen-atmosphere white dwarfs observed in Figure 11.

